Distributed Synthesis of Surveillance Strategies for Mobile Sensors

We study the problem of synthesizing strategies for a mobile sensor network to conduct surveillance in partnership with static alarm triggers. We formulate the problem as a multi-agent reactive synthesis problem with surveillance objectives specified as temporal logic formulas. In order to avoid the state space blow-up arising from a centralized strategy computation, we propose a method to decentralize the surveillance strategy synthesis by decomposing the multi-agent game into subgames that can be solved independently. We also decompose the global surveillance specification into local specifications for each sensor, and show that if the sensors satisfy their local surveillance specifications, then the sensor network as a whole will satisfy the global surveillance objective. Thus, our method is able to guarantee global surveillance properties in a mobile sensor network while synthesizing completely decentralized strategies with no need for coordination between the sensors. We also present a case study in which we demonstrate an application of decentralized surveillance strategy synthesis.

==> contracts.tex <==
%\subsection{Overview}
%We first provide an informal high level overview of the solution. We decentralize the synthesis process by solving each of the subgames separately. However, for a controller to be realizable, the sensors need to be aware of when targets are about to enter their region. To enforce this, we make use of \emph{static} sensors that can detect if a target has entered a particular set of states - though it cannot specify exactly which state the target is in. Informally
%
%\subsection{Border states}
%We say a state $l_t \in \widetilde{L}$ is a \emph{border state} of the surveillance subgame $G^i$ for sensor $i$ if $((l_i,l_t),(l_i',k_i)) \in \widetilde{T}_i$. Intuitively, if the target can exit the states of the subgame, i.e, it can enter $L\setminus\widetilde{L}_i$, then the state is known as a border state. We define the set of such states as the \emph{bordering set} $C_i$ of subgame $G^1_{\tilde{S}}$. 
%
%We extend this definition to the belief subgame $G^i_{\tilde{S}_\belief}$ by saying $B_t$ is a \emph{belief border state} for sensor $i$ if $((l_i,B_t),(l_i',B_t')) \in \widetilde{T}_i$ and $B_t \cap C_i \neq \emptyset$ 
%
%\begin{example}
%In Figure \ref{part-grid}, $C_1 = \{10,14\}$. \qed
%\end{example}
%
%\subsection{Neighbouring subgames}
%We say subgames $G^i$ and $G^j$ are \emph{neighbouring} if in the global game $G$ there exists a transition from $S_i$ to $S_j$ and vice versa (we assume with loss of generality that if there exists a transition from $s$ to $s'$ then the backwards transition must also exist). More formally if there exists transition $((l_i,l_t),(l_i',l_t')) \in T$ such that $l_t \in \widetilde{L}_i$ and $l_t' \in \widetilde{L}_j$, then $G^i$ and $G^j_{\tilde{S}}$ are \emph{neighbouring subgames}.
%
%\begin{proposition}
%If $G^i$ and $G^j$ are \emph{neighbouring} subgames then exists a transition $((l_i,l_t),(l_i',l_t')) \in T$ such that $l_t \in C_i$ and $l_t' \in C_j$. We denote the set of states satisfying this $C_{i \rightarrow j} \subseteq C_i$.
%\end{proposition}
%
%Simply, if two subgames are neighbours then there must exist a way to move from the border states of one to the border states of the other. 
%
%\subsection{Contracts between subgames}
%In order for a sensor to be able to react to surveillance targets in its subgame, it is necessary for it to be made aware when a target has moved into its subgame. We enforce this assumption in the form of a \emph{contract} between neighbouring subgames. To do this, in each subgame $G^i$ we augment boolean variables $c_{ij}$ to the state where $c_{ij} = \true$ if $l_t \in C_{j \rightarrow i}$. Intuitively, $c_{ij}$ evaluating to $\true$ is sensor $j$ letting sensor $i$ know that it is possible for the target to enter the state space of subgame $G^i$. 
%\begin{example}
%Referring to Figure \ref{part-grid}, the new augmented state with the contract variable for $G^2$ is $s_2 = (4,k_2,\true)$. From this state, sensor $2$ is aware that the target can transition into $\widetilde{L}_2$ in the next step. The only possible transitions from $(l_2,k_2, \false)$ is $(l_2',k_2, \true)$ and $(l_2',k_2, \false)$. In other words the target cannot transition into $\widetilde{L}_2$ from a non-border state. 
%\end{example}

==> figs/simple-belief-transitions.tex <==
\begin{center}
\begin{tikzpicture}[node distance=.9 cm,auto,>=latex',line join=bevel,transform shape,scale=.75]
\node at (0,0) (s0) {$((20,4),\{18\})$};
\node  [below left of=s0,yshift=-.5cm,xshift=-0.5cm] (s2) {$((15,3),\{19,23\})$};
\node  [below right of=s0,yshift=-.5cm,xshift=1cm] (s3) {$((15,3),\{19,23\})$};
\node  [left of=s2,xshift=-2cm] (s1) {$((21,9),\{19,23\})$};
\node  [right of=s3,xshift=2cm] (s4) {$((21,9),\{17\})$};
\draw [->] (s0) edge (s1.north);
\draw [->] (s0) edge (s2.north);
\draw [->] (s0) edge (s3.north);
\draw [->] (s0) edge (s4.north);
\end{tikzpicture}
\end{center}


==> synthesis.tex <==
We are now ready to solve each game $G^i$ with local surveillance objective $\locspec_i$. However, for a controller to 
